Bootstrapping Relation Extractors using Syntactic Search by Examples

The advent of neural-networks in NLP brought with it substantial improvements in supervised relation extraction. However, obtaining a sufficient quantity of training data remains a key challenge. In this work we propose a process for bootstrapping training datasets which can be performed quickly by non-NLP-experts. We take advantage of search engines over syntactic-graphs (Such as Shlain et al. (2020)) which expose a friendly by-example syntax. We use these to obtain positive examples by searching for sentences that are syntactically similar to user input examples. We apply this technique to relations from TACRED and DocRED and show that the resulting models are competitive with models trained on manually annotated data and on data obtained from distant supervision. The models also outperform models trained using NLG data augmentation techniques. Extending the search-based approach with the NLG method further improves the results.

==> figures/neg_ratios_on_children.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{plots/children_plot.pdf}
\caption{TACRED's \textit{per:children} relation, experimenting with different ratios and types of negative examples. 47 represent the ratio as seen in development set.}
\label{fig:children_negatives}
\end{figure}

==> tables/f1_per_relation.tex <==
\begin{table}[t]
\begin{tabular}{l|ccc}
Relation            & P & R & F1 \\
\hline
org:country\_of\_hq & 0.608                 & 0.522                 & 0.557                  \\
org:founded\_by     & 0.668                 & 0.828                 & 0.738                  \\
per:children        & 0.483                 & 0.505                 & 0.493                  \\
per:city\_of\_death & 0.867                 & 0.262                 & 0.398                  \\
per:date\_of\_death & 0.623                 & 0.611                 & 0.612                  \\
per:origin          & 0.713                 & 0.523                 & 0.597                  \\
per:religion        & 0.610                 & 0.383                 & 0.469                  \\
per:spouse          & 0.737                 & 0.662                 & 0.688                  \\
\hline
Average             & 0.664                 & 0.537                 & 0.569
\end{tabular}
\caption{Overall Precision, Recall and F1 for per relation on \tacred}
\label{table:f1_per_relation}
\end{table}

==> tables/multiclass.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|c|c}
{\textbf{Relation}} & {\textbf{Multi Class}} & {\textbf{Binary}}\\
\hline
{org:country\_of\_hq} & {0.380} & {0.557}\\
{org:founded\_by} & {0.698} & {0.737}\\
{per:children} & {0.438} & {0.493}\\
{per:city\_of\_death} & {0.450} & {0.398}\\
{per:date\_of\_death} & {0.629} & {0.617}\\
{per:origin} & {0.604} & {0.597}\\
{per:religion} & {0.553} & {0.469}\\
{per:spouse} & {0.617} & {0.688}\\
\hline
{Average} & {0.546}  & {0.569}\\
\end{tabular}
\caption{F1 comparison between relation extractor performance over selected relations in multi-class and binary classification settings. Multi Class's F1 score over all relation in \tacred~is $0.652$}
\label{tab:multivsbinary}
\end{table}

==> tables/neg_patterns.tex <==
\begin{longtable}{| p{\textwidth} |}
\endfirsthead
\hline
\endfirsthead
\endhead
\multicolumn{1}{r}{\textit{Continued on next page}} \\
\endfoot
\endlastfoot
\hline
\textbf{Sentences with 2 Person mentions} \\
! (?<e1>[entity=PERSON]+) [entity!=PERSON]+ (?<e2>[entity=PERSON]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Person and Date mentions} \\
! (?<e1>[entity=PERSON]+) []+ (?<e2>[entity=DATE]+) \#e e1 e2 \\
! "(?<e1>[entity=DATE]+) []+ (?<e2>[entity=PERSON]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Organization and Date mentions} \\
! (?<e1>[entity=ORGANIZATION]+) []+ (?<e2>[entity=DATE]+) \#e e1 e2 \\
! "(?<e1>[entity=DATE]+) []+ (?<e2>[entity=ORGANIZATION]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Organization and Person mentions} \\
! (?<e1>[entity=ORGANIZATION]+) []+ (?<e2>[entity=PERSON]+) \#e e1 e2 \\
! "(?<e1>[entity=PERSON]+) []+ (?<e2>[entity=ORGANIZATION]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Organization and Location mentions} \\
! (?<e1>[entity=ORGANIZATION]+) []+ (?<e2>[entity=LOCATION]+) \#e e1 e2 \\
! "(?<e1>[entity=LOCATION]+) []+ (?<e2>[entity=ORGANIZATION]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Person and Location mentions} \\
! (?<e1>[entity=PERSON]+) []+ (?<e2>[entity=LOCATION]+) \#e e1 e2 \\
! "(?<e1>[entity=LOCATION]+) []+ (?<e2>[entity=PERSON]+) \#e e1 e2" \\
\hline
\textbf{Sentences with Person and Misc mentions} \\
! (?<e1>[entity=PERSON]+) []+ (?<e2>[entity=MISC]+) \#e e1 e2 \\
! "(?<e1>[entity=MISC]+) []+ (?<e2>[entity=PERSON]+) \#e e1 e2" \\
\hline
\caption{Negative examples SPIKE patterns}
\label{tab:negative_patterns}
\end{longtable}

==> tables/scores_table_gen.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|c|c}
{\textbf{Method}}               & \textbf{TACRED}  & \textbf{DocRED} \\ 
\hline
{Example Generation}                   & {0.439} & {0.109} \\ 
{Search + Generation}    & {0.491} & {0.277} \\ 
\end{tabular}
\caption{Average test F1 score over generative based methods.}
\label{tab:f1_table_gen}
\end{table}

==> tables/scores_table_syn_search.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|c|c}
{\textbf{Method}}               & \textbf{TACRED}  & \textbf{DocRED} \\ 
\hline
{Annotated - 5+50}                & {0.097} & {0.140} \\ 
{Annotated - 10+100}               & {0.136} & {0.215} \\ 
{Annotated - 20+200}               & {0.266} & {0.271} \\ 
{Annotated - 50+500}               & {0.458} & {0.311} \\ 
{Annotated - 100+1000}              & {0.516} & {0.321} \\ 
{Annotated - All}              & {0.569} & {0.306} \\ 
\hline
{Pattern Based RE}   & {0.128} & {-}     \\
\hline
{Synt. Search}       & {0.443} & {0.266} \\
\end{tabular}
\caption{Average test F1 score over all relations. Synt. Search row is trained on data created from 3 annotated patterns. The Annotated experiments are denoted by the number of positive examples + negative examples.}
\label{tab:f1_table}
\end{table}

==> tables/size_distant.tex <==
@@I don't use this
\begin{table}[t]
\centering
\begin{tabular}{l|c|c}
{\textbf{Method}}               & \textbf{DocRED} \\ 
\hline
{Distant Sup. - 100}    & {0.262}     \\
{Distant Sup. - 500}    & {0.314}     \\
{Distant Sup. - 1000}   & {0.312}     \\
\end{tabular}
\caption{}
\label{tab:size_distant}
\end{table}
